Learning Robust Low-Rank Representations

In this paper we present a comprehensive framework for learning robust low-rank representations by combining and extending recent ideas for learning fast sparse coding regressors with structured non-convex optimization techniques. This approach connects robust principal component analysis (RPCA) with dictionary learning techniques and allows its approximation via trainable encoders. We propose an efficient feed-forward architecture derived from an optimization algorithm designed to exactly solve robust low dimensional projections. This architecture, in combination with different training objective functions, allows the regressors to be used as online approximants of the exact offline RPCA problem or as RPCA-based neural networks. Simple modifications of these encoders can handle challenging extensions, such as the inclusion of geometric data transformations. We present several examples with real data from image, audio, and video processing. When used to approximate RPCA, our basic implementation shows several orders of magnitude speedup compared to the exact solvers with almost no performance degradation. We show the strength of the inclusion of learning to the RPCA approach on a music source separation application, where the encoders outperform the exact RPCA algorithms, which are already reported to produce state-of-the-art results on a benchmark database. Our preliminary implementation on an iPad shows faster-than-real-time performance with minimal latency.

==> input_experiments.tex <==
\section{Experimental results}
\label{sec.experiments}


%
%We henceforth refer as \emph{Exact} to the representation obtained using Algorithm~\ref{alg:so} with $\bb{U}$ computed from the training data using SVD. Unless specified otherwise, the upper bound of %the rank was set to $q = 50$.

%to the neural network sparse encoders obtained by minimizing Gregor\&LeCun's objective function, this is, the $\ell_2$ discrepancy with the output of the exact encoder. It will be explicitly stated when neural network sparse encoders are trained using a specific objective function (e.g., \emph{NN Lasso}).

Two datasets were used in the experiments: The \emph{faces} dataset consisted of $800$ $66 \times 48$ images of a female face photographed over the timespan of $4.5$ years, roughly pose- and scale-normalized and aligned.\footnote{The original video can be found at {\footnotesize\texttt{http://www.youtube.com/watch?v=02e5EWUP5TE}}.} The surveillance sequence ``\emph{Hall of a business building}'' taken from \cite{Li04statisticalmodeling} consisted of $88 \times 72$ images of an indoor scene shot by a static camera in a mall. The scene has a nearly constant background and walking people in the foreground.
We used $q=50$ and $\lambda_\ast=0.1$ and $\lambda = 10^{-2}$

\begin {table}[tb]
\caption{Robust PCA representation accuracy (in the sense of the $\ell_2+\ell_1$ cost) of the faces data using different encoders. The cost for the exact encoder is $1.290$. \label{tab:faces} }
\begin{center}
\begin{tabular}{lcccccccc}
  \hline\hline
\multirow{2}{*}{\textbf{Encoder}}      &\hspace{5mm} & \multirow{2}{*}{\textbf{Untrained}} &\hspace{5mm} &\multirow{2}{*}{\textbf{Approx.}} &\hspace{5mm}  & \multirow{2}{*}{\textbf{$\ell_2 + \ell_1$}} & \hspace{5mm} & \textbf{$\ell_2 + \ell_1$ with} \\
                                       & &                                    & &                               & &                                            & & \textbf{$\bb{U}$ update} \\
\hline
\textbf{Single layer}   & &  1.3355	& & 1.3471    & &	1.3460 & &   	1.3262 \\
\textbf{$(2,10)$ layers}   & &  (1.325,1.297)	& & (1.326,1.298)   & &	(1.325,1.297) & &  (1.317,1.288) \\
%\textbf{$2$ layers}   & &  1.3248	& & 1.3261    & &	1.3255 & &   	1.3171 \\
%\textbf{$5$ layers}   & &  1.3073	& & 1.3085    & &	1.3078 & &   	1.2995 \\
%\textbf{$10$ layers} & &  1.2968	& & 1.2977	& &   1.2969 & &   	1.2885 \\
%\hline
%\textbf{Exact} & & \multicolumn{7}{c}{1.2903} \\
  \hline\hline
\end{tabular}
\end{center}
\vspace{-3ex}
\end{table}

\begin{figure}
\vspace{-2ex}
\begin{centering}
\includegraphics[width=0.5\linewidth]{online_cost2.eps}
\vspace{-1mm}
\caption{Performance, in the sense of the cost \eqref{ec.convex.unconstrained}, of the online and offline encoders on the faces sequence. Representative faces
are also shown.  \label{fig:online} }
%\vspace{-1ex}
\end{centering}
\end{figure}
\begin{figure}[t]
%\vspace{-1ex}
\includegraphics[width=\linewidth]{geometric1.eps}
\vspace{-1mm}
\caption{Robust PCA representation of the faces dataset in the presence of geometric transformations (misalignment).
Left group: original faces; middle group: shifted faces; right group: faces optimally realigned during encoding.
First row: reconstructed face $\bb{Us}+\bb{o}$; middle row: its low-rank approximation $\bb{Us}$; and bottom row: sparse outlier $\bb{o}$.
The $\ell_2+\ell_1$ cost is given for each representation.
 \label{fig:geometric} }
\vspace{-3ex}
\end{figure}
%\vspace{-1ex}


\mypara{Coding performance} In order to evaluate the quality of different robust PCA encoders, neural networks with different number of layers were trained on $500$ vectors from the faces dataset. The following training objectives were used: the $\ell_2$ discrepancy between the exact representation $\bb{s}$ and $\bb{o}$ (denoted as \emph{Approx.});
the $\ell_2+\ell_1$ objective; and the $\ell_2+\ell_1$ objective combined with the online update of the dictionary $\bb{U}$ (initial dictionary was computed using standard SVD).
For reference, we also report the results produced by the exact Algorithm~\ref{alg:so}, and an \emph{untrained} network with $\bb{W}$, $\bb{H}$ and $\bb{\lambda}$ initialized according to Algorithm~\ref{alg:so} (being effectively a truncated version of the algorithm).
%
The obtained representations are visualized in Figure~\ref{fig:face-reconst}. Table~\ref{tab:faces} summarizes the quality of the representations in terms of the $\ell_2+\ell_1$ cost (lower numbers correspond to better quality). Note how sufficiently deep encoders with dictionary update slightly outperform the exact encoder without dictionary adaptation. Also note that using a neural network encoder to approximate the exact representations slightly degrades the $\ell_2+\ell_1$ measure compared to the untrained encoder.



\mypara{Online learning} In this experiment we evaluate the online learning capabilities of the proposed neural network encoders.
As the input data we used the time-ordered sequence of $800$ images from the faces dataset.
%
Online learning was performed in overlapping windows of $100$ images with a step of $10$ images. We compared the exact algorithm,
a five layer neural network encoder trained offline using the $\ell_2 + \ell_1$ objective (\emph{NN offline}), and the same encoder trained online with adaptive $\bb{U}$.
The dictionary was initialized using SVD.
%
Performance measured in terms of the exact cost (\ref{ec.convex.unconstrained}) is reported in Figure~\ref{fig:online}. The exact offline encoder is consistently slightly inferior to the exact algorithm. However, thanks to its capabilities to adapt to the changing data distribution, the online encoder starts outperforming the offline counterparts after a relatively brief period of initial adaptation.

\mypara{Geometric transformations} We now evaluate the representation capabilities of the proposed neural network encoder in the presence of geometric transformations. A five layer encoder was trained on $600$ images from the faces dataset. As the test set, we used the remaining $200$ faces, as well as a collection of geometrically transformed images from the same test set. Sub-pixel planar translations were used for geometric transformations.
%
The encoder was applied to the misaligned set, optimizing  the $\ell_2+\ell_1$ objective over the transformation parameters.
For reference, the encoder was also applied to the transformed and the untransformed test sets without performing optimization.
%
Examples of the obtained representations are visualized in Figure~\ref{fig:geometric}.
%
Note the relatively larger magnitude and the bigger active set of the sparse outlier vector $\bb{o}$ produced for the misaligned faces, and how they are re-aligned when optimiziation over the transformation is allowed. Since the original data are only approximately aligned, performing optimal alignment during encoding frequently yields lower cost compared to the plain encoding of the original data.


\mypara{Video separation}  Figure~\ref{fig:surveillance} shows background and foreground separation via robust PCA on the surveillance video sequence ``\emph{Hall of a business building}'' taken from \cite{Li04statisticalmodeling}. The sequence consists of $88 \times 72$ images of an indoor scene shot by a static camera in a mall. The scene has a nearly constant background and walking people in the foreground. We used networks with five layers and $q=5$ %$\lambda_\ast=0.1$, $\lambda = 10^{-3}$
trained to approximate the output of the exact RPCA on a subset of the frames in the sequence.
The separation produced by the fast encoder is nearly identical to the output of the exact algorithm and to the output of the code from \cite{Lin2009-pp}, used as reference, while being considerably faster.
%
Our Matlab implementation with built-in GPU acceleration executed on an NVIDIA Tesla C2070 GPU propagates of an image through a single layer of the network in merely $92\mu sec$. This is several orders of magnitude faster than the commonly used iterative solver executed on the CPU.

\begin{figure}[t]
\includegraphics[width=\linewidth]{surveillance2.eps}
\vspace{-1mm}
\caption{Robust PCA representation of several frames from the surveillance sequence
obtained using the algorithm in \cite{Lin2009-pp} (left group), Algorithm~\ref{alg:so} (middle group), and a five layer neural network encoder (right group). Columns in each group are, left-to-right: the reconstructed frame $\bb{Us}+\bb{o}$, its low-rank approximation $\bb{Us}$ (background), and the sparse outlier $\bb{o}$ (foreground). Each row corresponds to a different frame.
\label{fig:surveillance} }
\vspace{-3ex}
\end{figure}

\mypara{Audio separation} We evaluate the separation performance of the proposed methods on the MIR-1K dataset \cite{hsu2010improvement}, containing $1000$ $16$ KHz clips extraced from $110$ Chinese karaoke songs performed by $19$ amateur singers ($11$ males and $8$ females).
Each clip duration ranges from $4$ to $13$ seconds, totaling about $133$ minutes.
We reserved about $23$ minutes of audio sang by one male and one female singers (\emph{abjones} and \emph{amy}) for the purpose of training; the remaining $110$ minutes
of $17$ singers were used for testing. The voice and the music tracks were mixed linearly with equal energy.

The experimental settings closely followed that of \cite{hsu2010improvement}, to which the reader is referred for further details.
As the evaluation criteria, we used the standard BSS-EVAL metrics \cite{vincent2006performance}, which calculate the \emph{source-to-distortion ratio} (SDR), the \emph{source-to-artifacts ratio} (SAR), and the \emph{source-to-interference ratio} (SIR).
%
Following \cite{huang12}, we computed the global normalized SDR, %\footnote{In general, the prefix ``G'' indicates when the measure is averaged throughout the sample,e.g. GSAR.}
$\mathrm{GNSDR} = \sum_{i=1}^{N} \delta_i (\mathrm{SDR}(\hat{s},s)-\mathrm{SDR}(x,s))$,
where $\hat{s}$ and $s$ are the corresponding original and estimated voice signal, $x$ is the mixture, $\delta_i$ is the relative duration of each of the $N$ pieces.
We also computed the \emph{signal-to-noise ratio} (SNR), with the ground-truth being the signal,
and the difference between the ground-truth and the reconstructed signal being the noise.
%

All networks used $20$ layers with $q=25$. The following training regimes were compared: untrained parameters initialized according to Algorithm~\ref{alg:so} (\emph{Untrained});
unsupervised learning with the objective (\ref{ec.robust.projection}) (\emph{Unsupervised});
and training supervised by the clean voice and background tracks (\emph{Supervised}).
%
For reference, we also give results of ideal frequency masking as well as that of two exact RPCA algorithm minimizing (\ref{ec.convex.unconstrained}) using proximal splitting,
and its noiseless version using augmented Lagrangian.
%
Table~\ref{tab:comparison} summarizes the obtained separation performance. While unsupervised training makes fast RPCA encoders on par
with the exact RPCA (at a fraction of the computational complexity and latency of the latter), significant improvement is achieved by using the supervised regime.
%
We intend to release a demo iOS application capable of performing the separation online and in real-time on a hand-held device.


\begin {table}[tb]
\caption{\small{Performance of audio separation methods on the MIR-1K dataset.} \label{tab:comparison} }
\begin{center}
%\begin{tabular}{lcccccccc}
%  \hline\hline
%\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{GNSDR}} & \multicolumn{2}{c}{\textbf{GSNR}} & \multicolumn{2}{c}{\textbf{GSAR}} & \multicolumn{2}{c}{\textbf{GSIR}} \\
%                                 & \textbf{voice} & \textbf{music}    & \textbf{voice} & \textbf{music}   & \textbf{voice} & \textbf{music}   & \textbf{voice} & \textbf{music}   \\
\scriptsize{
\begin{tabular}{lcccc}
  \hline\hline
\textbf{Method} &  \textbf{GNSDR}  &  \textbf{GSNR}  &  \textbf{GSAR}  & \textbf{GSIR} \\
\hline
Ideal freq. mask          & 13.48         & 5.46             & 13.65                   & 31.22  \\
ADMoM RPCA \cite{huang12} &	5.00          & 2.38             & 6.68                    & 13.76  \\
%\hline
Proximal RPCA	          & 5.48          & 3.29             & 7.02                    & 13.91  \\
NN RPCA Untrained	      & 5.30          & 2.66             & 6.80                    & 13.00  \\
NN RPCA Unsupervised      & 5.62 	      & 2.87             & 6.90                    & 14.02  \\
NN RPCA Supervised        & 6.38          & 3.18             & 7.22                    & 16.47  \\
  \hline\hline
\end{tabular}
}
\end{center}
\vspace{-3ex}
\end{table} 

==> input_figure1.tex <==
\begin{figure*}[t]

\vspace{5mm}
\begin{center}
    \begin{overpic}
    [width=1\linewidth]{flow-diagrams.pdf}
   \scriptsize{
	\put(7,15.7){$\bb{x}\!\!-\!\!\bb{W}\!\bb{x}$}
	\put(86.05,6.95){$\bb{H}(\!\bb{x}\!\!-\!\!\bb{o}\!)$}
	   \put(26.5,0.5){Layer 1}
	   \put(64.8,0.5){Layer $T$}
   }
    \footnotesize{
    \put(24,32){$\bb{W}$}
    \put(33.5,32){$\bb{\lambda}$}


    \put(-1,17){$\datav$}

        \put(14.7,17.6){$\bb{b}_\mathrm{in}$}
    \put(14.7,8.5){$\bb{o}_\mathrm{in}$}

    \put(11.2,7){$\bb{0}$}



    \put(41,17.6){$\bb{b}_\mathrm{out}$}
    \put(41,8.6){$\bb{o}_\mathrm{out}$}

    \put(52.5,17.6){$\bb{b}_\mathrm{in}$}
    \put(52.5,8.6){$\bb{o}_\mathrm{in}$}

    \put(96,25.5){$\bb{o}$}
    \put(96,8.6){$\bb{s}$}

%    \put(88,13.2){$\bb{\pi}_{\bb{t}}$}
    \put(88.6,19.7){$\bb{H}$}

\put(21,15.5){$\bb{b}_\mathrm{out} \!= \bb{b}_\mathrm{in}\!\! +\!\ldots$}
\put(22.9,12){$\bb{W}(\!\bb{o}_\mathrm{out}\!-\!\bb{o}_\mathrm{in})$}
\put(21,7){$\bb{o}_\mathrm{out} = \bb{\pi}_{\bb{\lambda}}(\bb{b}_\mathrm{in})$}


\put(59.4,12.5){$\bb{o}_\mathrm{out} = \bb{\pi}_{\bb{\lambda}}(\bb{b}_\mathrm{in})$}


    \put(47.6,15.5){$\cdots$}
    \put(47.6,6.95){$\cdots$}

    }
    \end{overpic}
\end{center}
%\vspace{-2mm}
\caption{RPCA encoder architecture with $T$ layers. \label{fig:BCoFB}}
\end{figure*}

